Towards a Benchmarking Suite for Kernel Tuners

As computing system become more complex, it is becoming harder for programmers to keep their codes optimized as the hardware gets updated. Autotuners try to alleviate this by hiding as many architecture-based optimization details as possible from the user, so that the code can be used efficiently across different generations of systems. In this article we introduce a new benchmark suite for evaluating the performance of optimization algorithms used by modern autotuners targeting GPUs. The suite contains tunable GPU kernels that are representative of real-world applications, allowing for comparisons between optimization algorithms and the examination of code optimization, search space difficulty, and performance portability. Our framework facilitates easy integration of new autotuners and benchmarks by defining a shared problem interface. Our benchmark suite is evaluated based on five characteristics: convergence rate, local minima centrality, optimal speedup, Permutation Feature Importance (PFI), and performance portability. The results show that optimization parameters greatly impact performance and the need for global optimization. The importance of each parameter is consistent across GPU architectures, however, the specific values need to be optimized for each architecture. Our portability study highlights the crucial importance of autotuning each application for a specific target architecture. The results reveal that simply transferring the optimal configuration from one architecture to another can result in a performance ranging from 58.5% to 99.9% of the optimal performance, depending on the GPU architecture. This highlights the importance of autotuning in modern computing systems and the value of our benchmark suite in facilitating the study of optimization algorithms and their effectiveness in achieving optimal performance for specific target architectures.

==> content/method/framework.tex <==
\section{Autotuning framework}\label{sec:framework}
\begin{figure*}[]
    \centering
    \includegraphics[width=12cm]{content/method/experimental-pipeline.png}
    \caption{Experiment pipeline, including sample collection process and prediction stage.}
    \label{fig:experiment-pipeline}
\end{figure*}

In this section we will describe the implementation of our autotuning framework and techniques as illustrated in Fig.~\ref{fig:experiment-pipeline}.

\subsection{Measurement}
The total runtime of performing a computation on a GPU is heavily dependent on data transfer between the CPU's main memory and the GPUs memory via the PCIe-bus. Therefore, it is imperative that we first transfer the data and \emph{then} start the measurement timer when executing the kernel. Respectively, the timer needs to stop after the kernel has finished, but \emph{before} the data is transferred back to the host device. This ensures that we measure the actual execution time of the computation and not the additional time to transfer data between devices.



==> content/results/old_results.tex <==

\iffalse
\subsection{General data}

\subsubsection{TRIAD}
RTX 3060 (mobile GPU):
Speedup: 1.1325757575757576, AUC: 3.8050883717252955, Size: 4320
Budget: 5\%: 98.88\%, 1\%: 98.01\%
Performance: 99: 6.60\%, 95: 0.12\%, 90: 0.02\%

RTX 2080ti
Speedup: 1.2605346203824022, AUC: 9.130166796185486, Size: 4320
Budget: 5\%: 97.52\%, 1\%: 96.31\%
Performance: 99: 36.20\%, 95: 0.44\%, 90: 0.09\%

RTX 3090
Speedup: 1.5084852294154616, AUC: 12.061839024451928, Size: 4320
Budget: 5\%: 94.31\%, 1\%: 86.86\%
Performance: 99: 24.40\%, 95: 5.81\%, 90: 1.99\%

\subsubsection{nbody}
RTX 3060
Speedup: 1.7229189887641028, AUC: 5.636897553129544, Size: 1568
Budget: 5\%: 98.21\%, 1\%: 95.35\%
Performance: 99: 13.27\%, 95: 0.89\%, 90: 0.32\%

RTX 2080ti
Speedup: 1.371830088601378, AUC: 4.399785552731792, Size: 1568
Budget: 5\%: 98.76\%, 1\%: 97.34\%
Performance: 99: 7.91\%, 95: 0.45\%, 90: 0.26\%

RTX 3090
Speedup: 2.0267117362756717, AUC: 7.785006812164573, Size: 1568
Budget: 5\%: 97.00\%, 1\%: 91.78\%
Performance: 99: 17.60\%, 95: 2.30\%, 90: 0.70\%


\subsection{GEMM}
RTX 3060
Speedup: 15.839312509028312, AUC: 15.123815464017165, Size: 10306
Budget: 5\%: 90.52\%, 1\%: 71.88\%
Performance: 99: 16.38\%, 95: 8.03\%, 90: 4.79\%

RTX 2080ti
Speedup: 11.265880411738706, AUC: 3.5452133151132807, Size: 10306
Budget: 5\%: 99.92\%, 1\%: 89.17\%
Performance: 99: 2.59\%, 95: 1.51\%, 90: 1.05\%

RTX 3090
Speedup: 13.65917247896693, AUC: 3.9694728307040843, Size: 10306
Budget: 5\%: 99.83\%, 1\%: 88.82%
Performance: 99: 2.76\%, 95: 1.66\%, 90: 1.10\%

\subsubsection{hotspot}

RTX 3060
Speedup: 11.213062363151792, AUC: 3.0682773610278997, Size: 10000
Budget: 5\%: 99.33\%, 1\%: 98.14\%
Performance: 99: 2.43\%, 95: 0.55\%, 90: 0.36\%

RTX 2080Ti


RTX 3090
Speedup: 11.122751934021588, AUC: 5.401599185629197, Size: 10000
Budget: 5\%: 98.70\%, 1\%: 97.37\%
Performance: 99: 9.83\%, 95: 0.62\%, 90: 0.38\%

\fi


\subsection{Clustering analysis (t-sne)}
\begin{figure*}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{content/results/figures/t-sne/tsne_gemm_3090.png}  
  \caption{RTX 3090}
  \label{fig:facet_grid_median}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{content/results/figures/t-sne/tsne_gemm_3060.png}
  \caption{RTX 3060}
  \label{fig:facet_grid_cles}
\end{subfigure}\\
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{content/results/figures/t-sne/tsne_gemm_2080ti.png}
  \caption{RTX 2080ti}
  \label{fig:facet_grid_cles}
\end{subfigure}
\caption{t-SNE for GEMM on all architectures}
\label{fig:facet_grid}
\end{figure*}


\begin{figure*}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{content/results/figures/t-sne/tsne_hotspot_3090.png}  
  \caption{RTX 3090}
  \label{fig:facet_grid_median}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{content/results/figures/t-sne/tsne_hotspot_3060.png}
  \caption{RTX 3060}
  \label{fig:facet_grid_cles}
\end{subfigure}\\
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{content/results/figures/t-sne/tsne_hotspot_2080ti.png}
  \caption{RTX 2080ti}
  \label{fig:facet_grid_cles}
\end{subfigure}
\caption{t-SNE for hotspot on all architectures}
\label{fig:facet_grid}
\end{figure*}



\begin{figure*}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{content/results/figures/t-sne/tsne_nbody_3090.png}  
  \caption{RTX 3090}
  \label{fig:facet_grid_median}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{content/results/figures/t-sne/tsne_nbody_3060.png}
  \caption{RTX 3060}
  \label{fig:facet_grid_cles}
\end{subfigure}\\
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{content/results/figures/t-sne/tsne_nbody_2080ti.png}
  \caption{RTX 2080ti}
  \label{fig:facet_grid_cles}
\end{subfigure}
\caption{t-SNE for nbody on all architectures}
\label{fig:facet_grid}
\end{figure*}


\begin{figure*}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{content/results/figures/t-sne/tsne_triad_3090.png}  
  \caption{RTX 3090}
  \label{fig:facet_grid_median}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{content/results/figures/t-sne/tsne_triad_3060.png}
  \caption{RTX 3060}
  \label{fig:facet_grid_cles}
\end{subfigure}\\
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{content/results/figures/t-sne/tsne_triad_2080ti.png}
  \caption{RTX 2080ti}
  \label{fig:facet_grid_cles}
\end{subfigure}
\caption{t-SNE for TRIAD on all architectures}
\label{fig:facet_grid}
\end{figure*}

==> docsetup.tex <==
%\usepackage{setspace}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{color}
\usepackage{listings}
\usepackage{subcaption}
\usepackage{authblk}
\usepackage{xcolor}
\usepackage{mathtools}
\usepackage{mathptm}
\usepackage[T1]{fontenc}
\usepackage[pdftex,bookmarks=true]{hyperref}
\usepackage[pdftex]{hyperref}
\usepackage{float}

\usepackage{setspace}
\usepackage{enumitem}
\usepackage{booktabs}
%\usepackage[Lenny]{fncychap}
\usepackage{natbib}
\usepackage[font=small,labelfont=bf]{caption}
%\usepackage{fancyhdr}
\usepackage{times}

\usepackage[utf8]{inputenc}
\usepackage{babel}
\usepackage{textcomp}
\usepackage{type1cm}
\usepackage{amsfonts}
\let\labelindent\relax

\hypersetup{
    colorlinks,%
    citecolor=black,%
    filecolor=black,%
    linkcolor=black,%
    urlcolor=black
}
%\usepackage[font=small,labelfont=bf]{caption}
%\usepackage{fancyhdr}
%\usepackage{times}
%\usepackage[intoc]{nomencl}
%\renewcommand{\nomname}{List of Abbreviations}
%\makenomenclature
%\usepackage{natbib}
%\floatstyle{boxed} 
\restylefloat{figure}
\lstset{
    language=C,                             % Code langugage
    basicstyle=\ttfamily,                   % Code font, Examples: \footnotesize, \ttfamily
    keywordstyle=\color{OliveGreen},        % Keywords font ('*' = uppercase)
    commentstyle=\color{gray},              % Comments font
    numbers=left,                           % Line nums position
    numberstyle=\tiny,                      % Line-numbers fonts
    stepnumber=1,                           % Step between two line-numbers
    numbersep=5pt,                          % How far are line-numbers from code
    frame=none,                             % A frame around the code
    tabsize=2,                              % Default tab size
    captionpos=b,                           % Caption-position = bottom
    breaklines=true,                        % Automatic line breaking?
    breakatwhitespace=false,                % Automatic breaks only at whitespace?
    showspaces=false,                       % Dont make spaces visible
    showtabs=false,                         % Dont make tabls visible
    morekeywords={__global__, __device__},  % CUDA specific keywords
}

\definecolor{darkgreen}{rgb}{0.18,0.54,0.34}
\lstset{ 
  language=C,                % the language of the code
  basicstyle= \footnotesize,           % the size of the fonts that are used for the code
  numbers=left,
  numberfirstline=true,
  numbersep=5pt,                  % how far the line-numbers are from the code
  backgroundcolor=\color{white},      % choose the background color. You must add \usepackage{color}
  showspaces=false,               % show spaces adding particular underscores
  showstringspaces=false,         % underline spaces within strings
  showtabs=false,                 % show tabs within strings adding particular underscores
  frame=lrb,                   % adds a frame around the code
  rulecolor=\color{black},        % if not set, the frame-color may be changed on line-breaks within not-black text 
  tabsize=2,                      % sets default tabsize to 2 spaces
  captionpos=t,                   % sets the caption-position 
  breaklines=true,                % sets automatic line breaking
  breakatwhitespace=false,        % sets if automatic breaks should only happen at whitespace
  %title=\lstname,                   % show the filename of files included with \lstinputlisting;
  keywordstyle=\color{blue},          % keyword style
  commentstyle=\color{gray},       % comment style
  stringstyle=\color{darkgreen},         % string literal style
  escapeinside={\%*}{*)},            % if you want to add LaTeX within your code
  morekeywords={*, ..., __global__, __device__, threadIdx, method_t},               % if you want to add more keywords to the set
  xleftmargin=0.2in, % left horizontal offset of caption box
  xrightmargin=-.03in % right horizontal offset of caption box
}

% ShareLaTeX does not support glossaries now. Sorry...
%\usepackage[number=none]{glossary}
%\makeglossary
%\newglossarytype[abr]{abbr}{abt}{abl}
%\newglossarytype[alg]{acronyms}{acr}{acn}
%\newcommand{\abbrname}{Abbreviations} 
%\newcommand{\shortabbrname}{Abbreviations}
%%\makeabbr

